Neural Network-based Two-Dimensional Filtering for OTFS Symbol Detection

Orthogonal time frequency space (OTFS) is a promising modulation scheme for wireless communication in high-mobility scenarios. Recently, a reservoir computing (RC) based approach has been introduced for online subframe-based symbol detection in the OTFS system, where only the limited over-the-air (OTA) pilot symbols are utilized for training. However, the previous RC-based approach does not design the RC architecture based on the properties of the OTFS system to fully unlock the potential of RC. This paper introduces a novel two-dimensional RC (2D-RC) approach for online symbol detection on a subframe basis in the OTFS system. The 2D-RC is designed to have a two-dimensional (2D) filtering structure to equalize the 2D circular channel effect in the delay-Doppler (DD) domain of the OTFS system. With the introduced architecture, the 2D-RC can operate in the DD domain with only a single neural network, unlike our previous work which requires multiple RCs to track channel variations in the time domain. Experimental results demonstrate the advantages of the 2D-RC approach over the previous RC-based approach and the compared model-based methods across different modulation orders.

==> figures/fig_1d_rc_pre_process.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{fig_content/1d_rc_windowing.png}
% \vspace{-1.5em}
% \caption{Pre-processing steps of 1D RC.}
\caption{The windowing process in 1D-RC.}
\label{figs:1d_rc_pre_process}
\vspace{-1em}
\end{figure}

==> figures/fig_1d_rc_structure.tex <==
\begin{figure*}
\centering
\vspace{-1em}
\includegraphics[width=0.8\linewidth]{fig_content/1d_rc_structure_detail.pdf}
\caption{1D-RC Structure. For simplicity, the extended state and nonlinear function are ignored here. In the figure, the target output is a sequence with $N_o=1$. 
% The input, state, and output are colored in blue, green, and orange, respectively.
}
\label{figs:1d_rc_structure}
\vspace{-1em}
\end{figure*}

==> figures/figs_otfs_variants.tex <==
\begin{figure*}
\centering
\vspace{-1em}
\includegraphics[width=0.7\linewidth]{fig_content/otfs_variants.pdf}
% \vspace{-1.5em}
\caption{OTFS system variants.}
\label{fig:otfs_variants}
\vspace{-1em}
\end{figure*}

==> figures_results/fig_cp_otfs_rect.tex <==
\begin{figure*}
\centering%
% \vspace{-1em}
\subfloat[]{\label{a}\includegraphics[width=0.35\linewidth]{results/rc_rc_iir_ber_all_cp_otfs_10ns_qpsk.png}}%
\hspace{3em}
\subfloat[]{\label{b}\includegraphics[width=0.35\linewidth]{results/rc_rc_iir_ber_all_cp_otfs_10ns_16qam.png}}
%\vspace{-1em}
\caption{BER comparison in the CP-OTFS system.
(a) QPSK
(b) $16$ QAM
\label{figs:ber_cp_otfs}
}
% \vspace{-1em}
\end{figure*}

==> figures_results/fig_diff_velocity.tex <==
\begin{figure}
\centering
\vspace{-1em}
\includegraphics[width=0.8\linewidth]{results/ber_cp_otfs_10ns_qpsk_diff_speed.pdf}
% \vspace{-2em}
\caption{BER comparison with different velocities.}
\label{figs:ber_cp_qpsk_10ns_diff_velocities}
\vspace{-1em}
\end{figure}

==> figures_results/fig_ideal_pulse_int_delay_doppler.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{results/ber_ideal_pulse_int_delay_int_doppler_perfect_channel.png}
% \vspace{-2em}
\caption{BER comparison with ideal pulse shaping, perfect channel knowledge.}
\label{figs:ber_ideal_pulse_perfect_channel}
% \vspace{-1em}
\end{figure}

==> figures_results/fig_nmse_plots.tex <==
\begin{figure*}
\centering%
% \vspace{-1em}
\subfloat[]{\label{a}\includegraphics[width=0.3\linewidth]{results/train_nmse_Nn_window_size_rc_iir_cp_otfs.png}}%
\subfloat[]{\label{b}\includegraphics[width=0.3\linewidth]{results/test_nmse_Nn_window_size_rc_iir_cp_otfs.png}}
%\vspace{-1em}
\caption{Training and testing NMSE with different numbers of neurons and window sizes.
(a) Training NMSE
(b) Testing NMSE
\label{figs:train_test_nmse}
}
% \vspace{-1em}
\end{figure*}

==> figures_results/fig_otfs_16qam.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{results/ber_all_cp_rcp_otfs_10ns_16qam.png}
% \vspace{-2em}
\caption{BER comparison for $16$-QAM modulation.}
\label{figs:ber_rec_pulse_16qam_10ns}
% \vspace{-1em}
\end{figure}

==> figures_results/fig_otfs_qpsk.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{results/ber_all_cp_rcp_otfs_10ns_qpsk.png}
% \vspace{-2em}
\caption{BER comparison for QPSK modulation.}
\label{figs:ber_rec_pulse_qpsk_10ns}
% \vspace{-1em}
\end{figure}

==> figures_results/fig_rcp_otfs_rect.tex <==
\begin{figure*}
\centering%
% \vspace{-1em}
\subfloat[]{\label{a}\includegraphics[width=0.35\linewidth]{results/rc_rc_iir_ber_all_rcp_qpsk_10ns.png}}%
\hspace{3em}
\subfloat[]{\label{b}\includegraphics[width=0.35\linewidth]{results/rc_rc_iir_ber_all_rcp_16qam_10ns.png}}
%\vspace{-1em}
\caption{BER comparison in the RCP-OTFS system.
(a) QPSK
(b) $16$ QAM
\label{figs:ber_rcp_otfs}
}
% \vspace{-1em}
\end{figure*}

==> figures_results/fig_rcp_otfs_rect_16qam_10ns.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{results/rc_rc_iir_ber_all_rcp_16qam_10ns.pdf}
% \vspace{-2em}
\caption{BER comparison in the RCP-OTFS system under 16 QAM.}
\label{figs:ber_rcp_rec_pulse_16qam_10ns}
\vspace{-1em}
\end{figure}

==> figures_results/fig_rcp_otfs_rect_qpsk_10ns.tex <==
\begin{figure}
\centering
\vspace{-1em}
\includegraphics[width=0.8\linewidth]{results/rc_rc_iir_ber_all_rcp_qpsk_10ns.pdf}
% \vspace{-2em}
\caption{BER comparison in the RCP-OTFS system under QPSK.}
\label{figs:ber_rcp_rec_pulse_qpsk_10ns}
\vspace{-1em}
\end{figure}

==> figures_results/fig_test_nmse.tex <==
\begin{figure}
\centering
\vspace{-1em}
\includegraphics[width=0.8\linewidth]{results/test_nmse_Nn_window_size_rc_iir_cp_otfs.pdf}
% \vspace{-2em}
\caption{Testing NMSE with different numbers of neurons and window sizes.}
\label{figs:test_nmse}
\vspace{-1em}
\end{figure}

==> figures_results/fig_train_nmse.tex <==
\begin{figure}
\centering
\vspace{-1em}
\includegraphics[width=0.8\linewidth]{results/train_nmse_Nn_window_size_rc_iir_cp_otfs.pdf}
% \vspace{-2em}
\caption{Training NMSE with different numbers of neurons and window sizes.}
\label{figs:train_nmse}
\vspace{-1em}
\end{figure}

==> tables/CPU_runtime.tex <==
\begin{table}
\centering
% \footnotesize
\scriptsize
% \tiny
\vspace{-1em}
\caption{Average CPU run time of symbol detection algorithms}
\begin{tabular}{c c}
\toprule
% \hline
Method & Total processing time (Sec.) \\
\midrule
% \hline
% RCP-OTFS
% LMMSE &  6.24 \\
% \hline
% MPA & 128.66 \\
% \hline
% 1D RC & 2.20 \\
% \hline
% 2D RC & 1.99 \\
% CP-OTFS
% LMMSE & 5.29 \\
MPA & 99.33 \\
1D-RC & 2.12 \\
2D-RC & 1.98 \\
% \hline
\bottomrule
\end{tabular}
\vspace{-1em}
\label{tab:cpu_run_time}
\end{table}

==> tables/complexities.tex <==
\begin{table*}[!t]
\centering
% \scriptsize
\tiny
\vspace{-1em}
\caption{Computation Complexity}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{ c  c  c }
\toprule
% \hline
Method & Training\textbackslash{}Channel Estimation & Testing\textbackslash{}Equalization  \\
\midrule
% \hline
% LMMSE & $\mathcal{O}(|\Omega|)$ & $\mathcal{O}(M^3N^3)$ \\
% % \hline
% % Low complexity LMMSE & $\mathcal{O}(|\Omega|)$ & $\mathcal{O}(MN|\Omega|logN)$ \\
% % \hline
% % MRC & $\mathcal{O}(|\Omega|)$ & ${\mathcal O}(|L|N_{iter}NM)$\jiarui{double check if it is $1-\eta$ and add the number of iterations} \\
% MPA & $\mathcal{O}(|\Omega|)$ & $\mathcal{O}(N_{iter}|\Omega||\mathcal{A}|MN)$ \\
% % \hline
% % Multiple RC's & ${\mathcal O}(N_nNM+min\{(\eta MN/K)^2, N_n^2\}K)$ & ${\mathcal O}(N_nNM)$   \\
% 1D RC & $\mathcal{O}((N_i+N_n)(N_nMN +|\mathcal{L}_f||\Omega|^2/V+|\mathcal{L}_f||\Omega|))$ & $\mathcal{O}((N_n+N_i)MN)$   \\
% % \hline
% 2D RC & $\mathcal{O}(N_n(N_i+3N_n)MN + (N_n+N_i)(|\Omega|^2+|\Omega|)(|\mathcal{L}_{m}|+|\mathcal{L}_{n}|))$ & $\mathcal{O}((N_n+N_i)MN)$ \\
% % \hline

% LMMSE & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(M^3N^3)$ \\
% Low complexity LMMSE & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(\eta M^2N^2logN)$ \\
% MPA & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(\eta N_{iter}|\mathcal{A}|M^2N^2)$ \\
LMMSE & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(M^3N^3)$ \\
Low-complexity LMMSE & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(MN\tilde{P}logN)$ \\
MPA & $\mathcal{O}(\eta MN)$ & $\mathcal{O}(N_{iter}|\mathcal{A}|\tilde{P}MN)$ \\
1D-RC ($N_i+N_n \leq \eta MN/V$) & $\mathcal{O}(N_n(N_i+N_n)MN +(N_i+N_n)((\eta MN)^2/V+\eta MN)|\mathcal{L}_f|)$ & $\mathcal{O}((N_n+N_i)MN)$   \\
1D-RC ($N_i+N_n > \eta MN/V$) & $\mathcal{O}(N_n(N_i+N_n)MN + (N_i+N_n)((N_i+N_n)\eta MNV+\eta MN)|\mathcal{L}_f|)$ & $\mathcal{O}((N_n+N_i)MN)$   \\
2D-RC & $\mathcal{O}(N_n(N_i+3N_n)MN + (N_i+N_n)((\eta MN)^2+\eta MN)(|\mathcal{L}_{m}|+|\mathcal{L}_{n}|))$ & $\mathcal{O}((N_n+N_i)MN)$ \\

\bottomrule
\end{tabular}
% }
% \vspace{-2em}
\label{tab:complexity_table}
\end{table*}

% \begin{table*}[!t]
% \centering
% % \scriptsize
% % \tiny
% % \vspace{-1em}
% \caption{Computation Complexity}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcc}
% \toprule
% Method & Training\textbackslash{}Channel Estimation & Testing\textbackslash{}Equalization  \\
% \midrule
% LMMSE & $\mathcal{O}(|\Omega|)$ & $\mathcal{O}(MN|\Omega|logN)$ \\
% % MRC & $\mathcal{O}(|\Omega|)$ & ${\mathcal O}(|L|N_{iter}NM)$\jiarui{double check if it is $1-\eta$ and add the number of iterations} \\
% MPA & $\mathcal{O}(|\Omega|)$ & $\mathcal{O}(N_{iter}|\Omega||\mathcal{A}|MN)$ \\
% % Multiple RC's & ${\mathcal O}(N_nNM+min\{(\eta MN/K)^2, N_n^2\}K)$ & ${\mathcal O}(N_nNM)$   \\
% 1D RC & $\mathcal{O}((N_i+N_n)(N_nMN +L_f|\Omega|^2/V+L_f|\Omega|))$ & $\mathcal{O}((N_n+N_i)MN)$   \\
% 2D RC & $\mathcal{O}(N_n(N_i+3N_n)MN + (N_n+N_i)(|\Omega|^2+|\Omega|)(M_f+N_f))$ & $\mathcal{O}((N_n+N_i)MN)$ \\
% \bottomrule
% \end{tabular}
% % }
% % \vspace{-2em}
% \label{tab:complexity_table}
% \end{table*}

==> tables/exp_params.tex <==
\begin{table}[]
\centering
\caption{Simulation Parameters}
\begin{tabular}{lc}
\toprule
\textbf{Parameters of Wireless Channel} & \textbf{Values} \\
\midrule
% Channel Model & 3GPP 5G NR CDL, Rural Macro Scenario \\
Channel Model & 3GPP 5G NR CDL \\
Carrier frequency & 4 GHz       \\
Delay Profile in Channel Model & CDL-C \\
% Delay Spread & 10 ns \jiarui{change to 100 ns? other paper: 4$\mu s$}\\
% RMS Delay Spread & 10 ns \\
% Maximum Delay Spread & 87 ns \jiarui{change to 320 ns?}\\
Maximum Doppler Shift & 555 Hz\\
Carrier Spacing & 15 KHz \\
Sampling Rate & 15.36 MHz \\
Pilot Overhead for SISO & 4.69\% \\
$M$ & 1024 \\
$N$ & 14 \\
\bottomrule
% \textbf{Parameters of RC} & \textbf{Values} \\ \hline
% $L_{forget}$ & 22 \\ \hline
% $N_e$ & 8 $\sim$ 12\\ \hline
% $N_{skip}$ & 20 \\ \hline
% $p({\boldsymbol W}_{tran})$ & 0.7\\ \hline
% $r({\boldsymbol W}_{tran})$ & 0.8 \\ \hline
% $\sigma(\cdot)$ & $\arctan(\cdot)$ \\ \hline
% $\lambda$ & 10 \\ \hline
\end{tabular}
\label{tab:sim_para}
\end{table}


==> tables/notations.tex <==
\begin{table*}
\centering
\vspace{-1em}
% \scriptsize
\tiny
% \renewcommand{\arraystretch}{1.4}
\caption{Notations appearing in 2D-RC}
% \vspace{-2em}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ p{2.5cm} | p{5cm}}
\begin{tabular}{ l  l }
\toprule
% \hline
\textbf{Symbol} & \textbf{Definition} \\
\midrule
% \hline
$M_w$ & The window size along the delay dimension \\
% \hline
$N_w$ & The window size along the Doppler dimension \\
% \hline
% $\boldsymbol{Y}_{\mathrm{pad}} \in \mathbb{C}^{(M_w+M-1) \times (N_w+N-1)}$ & Zero-padded input used to form the windowed input \\
% \hline
$N_i$ & The input size to 2D RC \\
% \hline
$M_f$ & The maximum forget length along the delay dimension \\
% \hline
$N_f$ & The maximum forget length along the Doppler dimension \\
% \hline
$N_n$ & The number of neurons\\
% \hline
$\mathcal{L}_{m}$ & The delay forget length set with $M_f$ as the maximum delay forget length \\
% \hline
$\mathcal{L}_{n}$ & The Doppler forget length set with $N_f$ as the maximum Doppler forget length \\
% \hline
$m_f$ & The forget length in the delay forget length set $\mathcal{L}_{m}$\\
% \hline
$n_f$ & The forget length in the Doppler forget length set $\mathcal{L}_{n}$ \\
% \hline
$Y[l, k]$ & The ($l, k$)-th element of the received signal $\boldsymbol{Y}$ \\
$Y_c[l, k]$ & The ($l, k$)-th element of the phase compensated received signal $\boldsymbol{Y}_c$ \\
% \hline
$\hat{O}[m, n]$ & The estimated ($m, n$)-th output from 2D RC \\
% \hline
$\tilde{\bm{y}}[m, n]\in \mathbb{C}^{N_i}$ & The ($m, n$)-th element along the second and third dimensions of the input $\tilde{\mathbcal{Y}}$ \\
% \hline
$\bm{u}[m, n] \in \mathbb{C}^{N_n}$ & The state vector for the $(m, n)$-th input \\
% \hline
$\tilde{\bm{u}}[m, n] \in \mathbb{C}^{N_n+N_i}$ & The extended state of 2D RC \\
% \hline
$\bm{Y}_w[l, k] \in \mathbb{C}^{M_w \times N_w}$ & The windowing region for the input $Y[l, k]$ \\
$\bm{Y}_c \in \mathbb{C}^{M \times N}$ & The phase compensated received signal \\
% \hline
$\bm{W}_i \in \mathbb{C}^{N_n \times N_i}$ & The input weight matrix \\
% \hline
$\bm{W}_r \in \mathbb{C}^{N_n \times N_n}$ & The reservoir weight matrix along the row axis \\
% \hline
$\bm{W}_c \in \mathbb{C}^{N_n \times N_n}$ & The reservoir weight matrix along the column axis \\
% \hline
$\bm{W}_d \in \mathbb{C}^{N_n \times N_n}$ & The reservoir weight matrix along the diagonal axis \\
% \hline
$\bm{W}_o \in \mathbb{C}^{1\times (N_n+N_i)}$ & The output weight matrix \\
% \hline
$\hat{\bm{O}} \in \mathbb{C}^{(M + M_f) \times (N + N_f)}$ & The estimated output \\
% \hline
$\hat{\bm{O}}_{m_f, n_f} \in \mathbb{C}^{M \times N}$ & The truncated output with delay forget length $m_f$ and Doppler forget length $n_f$ \\
% \hline
$\bar{\bm{U}}_{m_f, n_f} \in \mathbb{C}^{(N_n+N_i) \times MN}$ & The masked truncated extended state matrix formed by vectoring $\bar{\mathbcal{U}}_{m_f, n_f}$ \\
% \hline
$\tilde{\bm{U}}_{\hat{m}_f, \hat{n}_f} \in \mathbb{C}^{(N_n+N_i) \times MN}$ & The truncated extended state matrix formed by vectoring $\tilde{\mathbcal{U}}_{\hat{m}_f, \hat{n}_f}$ \\
% \hline
$\hat{\bm{W}}_o^{(m_f, n_f)}$ & The trained output weights when utilizing delay forget length $m_f$ and Doppler forget length $n_f$ \\
% \hline
$\mathbcal{Y}_w \in \mathbb{C}^{N_i \times M \times N}$ & The 2D windowed input \\
% \hline
$\tilde{\mathbcal{Y}} \in \mathbb{C}^{N_i \times (M + M_f) \times (N + N_f)}$ & The 2D processed input to the 2D RC \\
% \hline
${\mathbcal{U}} \in \mathbb{C}^{N_n \times (M + M_f) \times (N + N_f)}$ & The state tensor \\
% \hline
$\tilde{\mathbcal{U}} \in \mathbb{C}^{(N_n+N_i) \times (M + M_f) \times (N + N_f)}$ & The extended state tensor \\
% \hline
$\tilde{\mathbcal{U}}_{m_f, n_f} \in \mathbb{C}^{(N_n+N_i) \times M \times N}$ & The truncated extended state tensor \\
% \hline
$\bar{\mathbcal{U}}_{m_f, n_f} \in \mathbb{C}^{(N_n+N_i) \times M \times N}$ & The masked truncated extended state tensor \\

\bottomrule
% \hline
\end{tabular}
% }
\label{tab:notations}
% \vspace{-2em}
\end{table*}
